MNN-AECS: Energy Optimization for LLM Decoding on Mobile Devices via Adaptive Core Selection

As the demand for on-device Large Language Model (LLM) inference grows, energy efficiency has become a major concern, especially for battery-limited mobile devices. Our analysis shows that the memory-bound LLM decode phase dominates energy use, and yet most existing works focus on accelerating the prefill phase, neglecting energy concerns. We introduce Adaptive Energy-Centric Core Selection (AECS) and integrate it into MNN to create the energy-efficient version, MNN-AECS, the first engine-level system solution without requiring root access or OS modifications for energy-efficient LLM decoding. MNN-AECS is designed to reduce LLM decoding energy while keeping decode speed within an acceptable slowdown threshold by dynamically selecting low-power CPU cores. MNN-AECS is evaluated across 5 Android and 2 iOS devices on 5 popular LLMs of various sizes. Compared to original MNN, MNN-AECS cuts down energy use by 23% without slowdown averaged over all 7 devices and 4 datasets. Against other engines, including llama.cpp, executorch, mllm, and MediaPipe, MNN-AECS delivers 39% to 78% energy saving and 12% to 363% speedup on average.

==> android-fixed.tex <==
\begin{table*}[!t]
    \centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccccccccccc}
    \toprule[1.5pt]
    \multirow{2}{*}{\bf device} & \multirow{2}{*}{\bf engine} & \multicolumn{3}{c}{\bf Qwen2.5-1.5B} & \multicolumn{3}{c}{\bf Qwen2.5-3B} & \multicolumn{3}{c}{\bf Llama3.2-1B} & \multicolumn{3}{c}{\bf Llama3.2-3B} & \multicolumn{3}{c}{\bf Gemma2-2B} \\
    \cmidrule(r){3-5}  \cmidrule(r){6-8}  \cmidrule(r){9-11}  \cmidrule(r){12-14} \cmidrule(r){15-17}
         & & {\bf speed} & {\bf battery} & {\bf energy} & {\bf speed} & {\bf battery} & {\bf energy} & {\bf speed} & {\bf battery} & {\bf energy} & {\bf speed} & {\bf battery} & {\bf energy} & {\bf speed} & {\bf battery} & {\bf energy} \\
    \midrule
    \multirow{6}{*}{Mate 40 Pro} & executorch & - & - & - & - & - & - & 11.5 & 44.5 & 639.7 & 4.6 & 109.2 & 1552.0 & - & - & - \\
	 & llama.cpp & 9.2 & 55.0 & 808.5 & 5.9 & 84.1 & 1179.3 & 14.4 & 39.8 & 562.5 & 5.5 & 87.4 & 1274.7 & - & - & - \\
	 & MediaPipe & - & - & - & - & - & - & - & - & - & - & - & - & 4.3 & 120.7 & 1700.2 \\
	 & mllm & 5.3 & 96.4 & 1376.0 & - & - & - & 5.3 & 90.5 & 1355.0 & - & - & - & - & - & - \\
	 & MNN & \textbf{19.4} & 30.7 & 426.3 & \textbf{10.0} & 53.1 & 805.0 & \textbf{24.8} & 22.5 & 340.1 & 9.1 & 59.1 & 858.5 & \textbf{11.5} & 46.3 & 715.9 \\
	 & ours & \underline{19.0} & \textbf{22.7} & \textbf{318.5} & \underline{9.8} & \textbf{48.1} & \textbf{708.0} & \underline{24.3} & \textbf{16.2} & \textbf{243.5} & \underline{\textbf{9.1}} & \textbf{45.9} & \textbf{669.0} & \underline{11.3} & \textbf{38.6} & \textbf{551.3} \\
	\midrule
	\multirow{6}{*}{V30 Pro} & executorch & - & - & - & - & - & - & 13.7 & 34.8 & 508.7 & 5.3 & 95.2 & 1326.6 & - & - & - \\
	 & llama.cpp & 9.0 & 49.2 & 743.7 & 6.0 & 80.7 & 1147.8 & 14.2 & 33.5 & 488.0 & 5.5 & 82.3 & 1231.8 & - & - & - \\
	 & MediaPipe & - & - & - & - & - & - & - & - & - & - & - & - & 4.6 & 95.6 & 1397.9 \\
	 & mllm & 6.2 & 81.0 & 1193.4 & - & - & - & 7.5 & 67.8 & 1031.7 & - & - & - & - & - & - \\
	 & MNN & \textbf{21.4} & 24.3 & 348.7 & \textbf{11.1} & 46.9 & 684.6 & \textbf{27.1} & 20.2 & 280.2 & \textbf{10.5} & 48.1 & 716.4 & \textbf{12.8} & 42.7 & 605.5 \\
	 & ours & 19.5 & \textbf{18.6} & \textbf{269.1} & \underline{10.2} & \textbf{35.9} & \textbf{518.3} & \underline{25.1} & \textbf{14.1} & \textbf{211.7} & \underline{9.9} & \textbf{36.5} & \textbf{546.7} & \underline{12.1} & \textbf{29.3} & \textbf{446.4} \\
	\midrule
	\multirow{6}{*}{Galaxy A56} & executorch & - & - & - & - & - & - & 14.0 & 30.4 & 453.8 & 5.7 & 75.2 & 1107.1 & - & - & - \\
	 & llama.cpp & 9.6 & 48.5 & 747.8 & 6.5 & 73.5 & 1097.2 & 15.1 & 32.4 & 502.4 & 6.0 & 76.3 & 1188.0 & - & - & - \\
	 & MediaPipe & - & - & - & - & - & - & - & - & - & - & - & - & 4.1 & 80.2 & 1204.1 \\
	 & mllm & - & - & - & - & - & - & 6.6 & 57.6 & 851.7 & - & - & - & - & - & - \\
	 & MNN & \textbf{17.3} & 22.3 & 332.3 & 8.6 & 42.8 & 628.8 & \textbf{21.2} & 18.0 & 262.3 & 8.2 & 43.9 & 692.3 & 10.0 & 35.8 & 565.9 \\
	 & ours & \underline{17.0} & \textbf{17.0} & \textbf{245.4} & \underline{\textbf{8.8}} & \textbf{31.3} & \textbf{472.5} & \underline{21.0} & \textbf{12.5} & \textbf{197.1} & \underline{\textbf{8.2}} & \textbf{33.0} & \textbf{505.6} & \underline{\textbf{10.0}} & \textbf{28.3} & \textbf{412.0} \\
	\midrule
	\multirow{5}{*}{Meizu 21} & executorch & - & - & - & - & - & - & 18.1 & 33.4 & 489.9 & 7.5 & 83.3 & 1184.3 & - & - & - \\
	 & llama.cpp & 10.6 & 62.4 & 909.0 & 7.0 & 95.7 & 1334.5 & 17.1 & 40.3 & 590.3 & 7.0 & 91.5 & 1397.7 & - & - & - \\
	 & mllm & - & - & - & - & - & - & 9.8 & 53.4 & 832.0 & - & - & - & - & - & - \\
	 & MNN & 20.3 & 22.4 & 329.5 & 10.9 & 41.7 & 638.9 & 25.3 & 16.8 & 250.9 & 10.6 & 44.0 & 672.7 & 10.2 & 45.0 & 701.3 \\
	 & ours & \underline{\textbf{23.1}} & \textbf{20.6} & \textbf{306.4} & \underline{\textbf{11.9}} & \textbf{36.0} & \textbf{551.9} & \underline{\textbf{28.5}} & \textbf{15.4} & \textbf{227.2} & \underline{\textbf{11.9}} & \textbf{41.4} & \textbf{632.0} & \underline{\textbf{10.5}} & \textbf{41.3} & \textbf{630.4} \\
	\midrule
	\multirow{6}{*}{Xiaomi 15 Pro} & executorch & - & - & - & - & - & - & 33.1 & 20.9 & 309.8 & 13.9 & 53.2 & 757.6 & - & - & - \\
	 & llama.cpp & 26.1 & 29.1 & 435.8 & 11.3 & 60.6 & 860.1 & 35.0 & 23.3 & 342.0 & 11.1 & 63.8 & 899.7 & - & - & - \\
	 & MediaPipe & - & - & - & - & - & - & - & - & - & - & - & - & 12.7 & 54.6 & 805.5 \\
	 & mllm & 11.7 & 51.5 & 787.4 & - & - & - & 14.1 & 43.0 & 671.6 & - & - & - & - & - & - \\
	 & MNN & 35.6 & 17.8 & 272.5 & 19.2 & 31.9 & 501.8 & 47.8 & 14.5 & 202.3 & 18.9 & 33.3 & 492.3 & 23.2 & 31.1 & 430.9 \\
	 & ours & \underline{\textbf{43.4}} & \textbf{14.5} & \textbf{211.3} & \underline{\textbf{23.2}} & \textbf{27.7} & \textbf{402.2} & \underline{\textbf{56.2}} & \textbf{12.3} & \textbf{173.0} & \underline{\textbf{22.3}} & \textbf{29.2} & \textbf{413.5} & \underline{\textbf{27.8}} & \textbf{22.2} & \textbf{348.7} \\
    \bottomrule[1.5pt]
    \end{tabular}
    }
    \caption{Android fixed length test results.}
    \label{tab:android-fixed}
\end{table*}

==> engine-model.tex <==
\begin{table}[!t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule[1.5pt]
          & Qwen2.5-1.5B & Qwen2.5-3B & Llama3.2-1B & Llama3.2-3B & Gemma2-2B \\
        \midrule
        executorch & \ding{53} & \ding{53} & \ding{52} & \ding{52}& \ding{53}\\
        llama.cpp & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\
        MediaPipe & \ding{53} & \ding{53} & \ding{53} & \ding{53} & \ding{52} \\
        mllm & \ding{52} & oom & \ding{52} & oom & \ding{53}\\
        MNN & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\
        ours & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Model compatibility of different engines on Android. \ding{52}, oom, and \ding{53} represents support, out of memory on some devices, and not supported.}
    \label{tab:engine-model}
\end{table}
